Flexibility Has a Price: Quantifying Modality Policies in Maliciously Secure Multi-Biometric Authentication

Multi-biometric authentication improves robustness and accessibility by combining information from multiple biometric modalities. Existing research has primarily focused on secure multimodal authentication, feature fusion, and recognition performance, while paying comparatively little attention to the security implications of modality-flexible authentication policies. At the same time, most systems provide limited cryptographic protection for biometric data during authentication. This paper addresses both challenges. We first study modality flexibility as a security decision rather than merely a usability feature. Each accepted modality subset creates an authentication entry point, and the resulting risk depends on the joint behavior of all accepted subsets and the attempt budget. We introduce a framework for quantifying this security cost and develop a policy-selection procedure that identifies policies satisfying a target risk level while supporting users who can present only a subset of modalities. We then present SUPERMBA, a two-server privacy-preserving authentication system that enforces the selected policy without revealing biometric templates or the modality subset used in an authentication attempt. The protocol provides verifiable policy enforcement even when one server is malicious and executes the same computation irrespective of the chosen policy or modality subset. Experiments on the three-modality MULB+ dataset show that allowing all modality subsets increases impostor risk from 1.21% for the weakest entry to 4.42% for the union of entries. On VidTIMIT, the increase is substantially smaller and is not statistically resolved with the available identities. SUPERMBA completes an authentication attempt in only 6.42 ms on MULB+ and 6.03 ms on VidTIMIT.

==> figs/system.tex <==
% v1/figs/system.tex -- participants, channels, and phases of \sysname (Figure in Sec. 4).
% Contains only the tikzpicture; \input inside a figure environment in sections/04-model.tex.
\begin{tikzpicture}[
  font=\footnotesize,
  >={Latex[length=4.5pt]},
  party/.style={draw, rounded corners=2pt, align=center, inner sep=3pt},
  srv/.style={draw, rounded corners=2pt, align=center, inner sep=2.5pt, minimum width=2.1cm},
  num/.style={circle, draw, inner sep=0.4pt, font=\tiny, fill=white},
  lbl/.style={font=\scriptsize, fill=white, inner sep=1pt, align=center},
]
% ---------- nodes ----------
\node[party, minimum height=1.9cm, text width=1.65cm] (client) at (-0.1,0)
  {\textbf{Client device} $\mathcal C$\\[3pt]
   {\scriptsize face, iris, hand}\\[2pt]
   {\scriptsize $e=\phi_S(x_S)$}};
\node[srv] (p0) at (3.5,0.74)
  {$\mathcal P_0$\\ {\scriptsize $[\![T_{u,k}]\!],[\![\hat\tau_{u,k}]\!],[\![\pi_{u,k}]\!]$}};
\node[srv] (p1) at (3.5,-0.74)
  {$\mathcal P_1$\\ {\scriptsize $[\![T_{u,k}]\!],[\![\hat\tau_{u,k}]\!],[\![\pi_{u,k}]\!]$}};
\node[draw, dashed, rounded corners=3pt, fit=(p0)(p1), inner sep=4pt] (srvbox) {};
\node[font=\scriptsize, below=1pt of srvbox] (cap) {$\le1$ corrupted, non-colluding};
\node[party, minimum height=1.9cm, text width=1.5cm] (sp) at (6.9,0)
  {\textbf{Service provider} $\mathcal{SP}$\\[3pt]
   {\scriptsize dealer}\\[1pt]
   {\scriptsize admission}\\[1pt]
   {\scriptsize decision}};
% ---------- online (solid) ----------
\draw[->] (client.east |- p0.west) -- node[lbl, above=1pt] {(3)\\ $\Delta_e,\Delta_{\boldsymbol\chi}$} (p0.west);
\draw[->] (client.east |- p1.west) -- (p1.west);
\draw[<->] (p0.south) -- node[lbl, right=1pt, font=\tiny, align=left] {(4) 2PC +\\MAC check} (p1.north);
\draw[->] (p0.east) -- node[lbl, above=1pt] {(5)\\ $\Delta_b,\Delta_{\alpha b}$} (sp.west |- p0.east);
\draw[->] (p1.east) -- (sp.west |- p1.east);
% ---------- offline / setup (dotted) ----------
\draw[->, dotted] (sp.north) |- ++(0,0.5) -| node[lbl, pos=0.25] {(1) correlated randomness} (srvbox.north);
\draw[->, dotted] ($(sp.north)+(0.35,0)$) |- ++(0,1.05) -| node[lbl, pos=0.25] {(2) input masks $\lambda_e,\lambda_{\boldsymbol\chi}$} (client.north);
% ---------- legend ----------
\draw[dotted, ->] (-1.1,-2.05) -- ++(0.55,0);
\node[font=\scriptsize, anchor=west] at (-0.5,-2.05) {preprocessing};
\draw[->] (1.3,-2.05) -- ++(0.55,0);
\node[font=\scriptsize, anchor=west] at (1.9,-2.05) {authentication};
\end{tikzpicture}


==> sections/A-proofs.tex <==
\section{Proofs}
\label{app:proofs}
% PURPOSE: proofs of the lemmas and of Theorem 1. May be moved to supplementary material.

\subsection{Proof of Lemma~\ref{lem:ip}}
Write $\bar X=\Delta_X+\delta_X$ and $\bar Y=\Delta_Y+\delta_Y$. By the definition of the offsets, $\bar X=X+\lambda_X+A_1-\lambda_X=X+A_1$ and $\bar Y=Y+B$. Summing the two servers' shares from step~1 of Figure~\ref{fig:ip} gives, for each coordinate $i$,
\[
\bar X_i\bar Y_i-A_{1,i}\bar Y_i-\bar X_iB_i+C_{1,i}=(\bar X_i-A_{1,i})(\bar Y_i-B_i)=X_iY_i,
\]
using $C_{1,i}=A_{1,i}B_i$. Hence $\Delta_z=\sum_iX_iY_i+\lambda_z$. The same computation with $\bar X'=\alpha X+A_2$ and $C_2=A_2\odot B$ gives $\Delta_{\alpha z}=\alpha\sum_iX_iY_i+\lambda_{\alpha z}$. All identities hold in $\mathbb Z_{2^{\ell+\sigma}}$. \hfill$\square$

\subsection{Public-Constant Multiplication}
For $\Delta_x=x+\lambda_x$, setting $\Delta_{cx}=c\Delta_x$ and $\lambda_{cx}=c\lambda_x$ gives $\Delta_{cx}-\lambda_{cx}=cx$. With $\lambda_{cx}=\lambda_x$ one obtains $cx+(c-1)\lambda_x$, which differs from $cx$ whenever $(c-1)\lambda_x\neq0$; exhaustive enumeration for $\ell\le6$ confirms that the failures are exactly these cases. Adding a public constant $c$ to an authenticated value maps the value component to $(\Delta_x+c,\langle\lambda_x\rangle)$ and the MAC component to $(\Delta_{\alpha x},\langle\lambda_{\alpha x}\rangle-c\langle\alpha\rangle)$, since $\alpha(x+c)=\alpha x+\alpha c$. \hfill$\square$

\subsection{Proof of Lemma~\ref{lem:cmp}}
Reduction modulo $2^\ell$ is a ring homomorphism from $\mathbb Z_{2^{\ell+\sigma}}$ to $\mathbb Z_{2^\ell}$, so $D=\Delta_z\bmod2^\ell=(\bar z+r)\bmod2^\ell$, where $\bar z=z\bmod2^\ell$ and $r=\lambda_z\bmod2^\ell$. Since $-2^{\ell-1}\le z<2^{\ell-1}$, we have $z\ge0$ iff $\bar z\in[0,2^{\ell-1}-1]$. Adding $r$ maps this interval to the cyclic interval from $p'=r$ to $q'=(2^{\ell-1}-1+r)\bmod2^\ell$. If $p'\le q'$, membership of $D$ in it is $\mathbf 1[D\le q']-\mathbf 1[D<p']$; if $p'>q'$, the interval wraps and membership is $\mathbf 1[D\ge p']+\mathbf 1[D\le q']=1-\mathbf 1[D<p']+\mathbf 1[D\le q']$. Both cases equal the right-hand side of Equation~\eqref{eq:ic}. The DCF keys output additive shares of $\mathbf 1[D<\gamma]\cdot(1,\alpha)$ for their points $\gamma$, and the dealer shares $\mathbf 1[p'>q']\cdot(1,\alpha)$; by linearity, the servers hold shares of $b\cdot(1,\alpha)$ with $b=\mathbf 1[z\ge0]$, and the output masks yield $\Delta_b-\lambda_b=b$ and $\Delta_{\alpha b}-\lambda_{\alpha b}=\alpha b$. \hfill$\square$

\subsection{Proof of Theorem~\ref{thm:main}}
\pending{To be checked line by line by the cryptography co-authors before submission.}

We describe the simulator $\mathsf{Sim}$ for a corrupted $\mathcal P_1$; the case of $\mathcal P_0$ differs only in which server adds the public product term in Figure~\ref{fig:ip}. $\mathsf{Sim}$ runs the adversary internally and plays $\mathcal F_{\mathsf{Prep}}$, the coin-tossing functionality, the honest server $\mathcal P_0$, the client, and $\mathcal{SP}$ toward it.

\emph{Simulation by execution on dummy inputs.} At enrollment, $\mathsf{Sim}$ chooses dummy templates (random unit vectors, encoded) for all $K$ slots and dummy thresholds and policy bits. On the admission metadata of an attempt, it chooses a dummy probe and a dummy slot index. It then generates all preprocessing exactly as $\mathcal F_{\mathsf{Prep}}$ would---including $\alpha$, every mask, and both DCF key pairs---and runs the code of the honest client, the honest server, and $\mathcal{SP}$ on the dummy inputs, interacting with the adversary. Because it generated all preprocessing and runs the honest parties, $\mathsf{Sim}$ knows every share and can compute, for every message the corrupted server sends, the message it should have sent. It records the difference.

\emph{Abort and output.} $\mathsf{Sim}$ runs $\Pi_{\mathsf{MAC}}$ and the release check of $\mathcal{SP}$ as written. If either fails, it sends \textsf{abort} to $\mathcal F_{\mathsf{Auth}}$. If both pass, it checks whether some recorded difference changes an opened value modulo $2^\ell$; if so it outputs \textsf{fail} (the bad event), and otherwise it lets $\mathcal F_{\mathsf{Auth}}$ deliver the decision on the real inputs to $\mathcal{SP}$.

\emph{The corrupted server's view.} We compare the view in the real execution with the view in the simulation through two hybrids. In the first, both key pairs of $\Pi_{\mathsf{Cmp}}$ are generated for an independent, uniformly random mask $r'$ in place of $r=\lambda_z\bmod2^\ell$, and the honest server evaluates its matching key. The honest server's key outputs enter the corrupted server's view only through the opening of $\Delta_b$ and $\Delta_{\alpha b}$, which are masked by fresh, uniform $\lambda_b$ and $\lambda_{\alpha b}$, and through the check values, which by the argument below depend only on the corrupted server's errors and $\alpha$; so the hybrid changes the view only through the corrupted server's own keys. A reduction to the security of the FSS scheme, which knows $r$ and $r'$ and can therefore produce $\Delta_z=z+r$ itself, shows that this costs at most $\mathrm{negl}(\kappa)$. Afterwards $r$ appears in the view only through $\Delta_z$, which is therefore uniform, and the keys have the same format for every mask (Section~\ref{ssec:blocks-cmp}). In the second hybrid, the honest inputs are replaced by the dummy inputs. Every public value that depends on an input is masked by a value that is uniform over $\mathbb Z_{2^{\ell+\sigma}}$, fresh for the attempt, used once, and of which the corrupted server holds only an additive share: the client's $\Delta_e$ and $\Delta_{\boldsymbol\chi}$; the operands $T_{u,k}+A_1^{(k)}$, $e+B$, and $\boldsymbol\chi+B'$; every opened $\Delta_x$ and $\Delta_{\alpha x}$, whose masks $\lambda_x$ and $\lambda_{\alpha x}$ are independent of each other and of all other masks. The public offsets are determined by these values and the public $\Delta$'s and add no information. The joint distribution of the public values together with the corrupted server's shares is therefore the same for any inputs, and the MAC relations hold in both hybrids because both execute the protocol honestly on some inputs. Templates are masked once at enrollment, and every attempt re-masks them with a fresh $A_1^{(k)}$, so the argument applies attempt by attempt.

\emph{The outcome.} Given the same view, both worlds abort exactly when $\Pi_{\mathsf{MAC}}$ or the release check fails. Suppose both pass. If no recorded difference changes an opened value modulo $2^\ell$, every value modulo $2^\ell$ equals its honest counterpart: differences in the upper $\sigma$ bits do not affect the comparison, which reads only the residue modulo $2^\ell$, nor any later product, because multiples of $2^\ell$ form an ideal; and a difference in the released $\Delta_b$ makes the servers' release messages differ or makes $b\notin\{0,1\}$, which $\mathcal{SP}$ rejects. By the argument at the end of Section~\ref{ssec:design-bitwidth}, $\mathcal{SP}$ then obtains the functionality's decision on the real inputs, as in the simulation. It remains to bound the bad event. The protocol verifies the scores before they are multiplied with $\boldsymbol\chi$ (Section~\ref{ssec:design-rationale}), and every other opened value is used afterwards only in local operations or as the input of $\Pi_{\mathsf{Cmp}}$, whose output is checked separately. An error therefore never reaches a check after having been multiplied by secret data, and the deviations visible to each check are the corrupted server's own: if it adds $e$ to an opened $\Delta_x$ and $e'$ to $\Delta_{\alpha x}$, the check value of the pair is $e'-\alpha e$, independent of the inputs. This is the expression analyzed for the batch check of SPDZ$_{2^k}$, where errors on an opened value and its MAC enter in exactly this form, and an offset the corrupted server adds to its share of the combined check value enters additively as there; the coefficients are drawn after all openings are fixed, and the commitments prevent the corrupted server from choosing its share of the combined check value after seeing the honest one. The analysis of~\cite{cramer2018spd} therefore bounds the probability that the check passes although some error is nonzero modulo $2^\ell$ by $\epsilon_{\mathrm{mac}}(\sigma)$. The digest prevents the client's inputs from differing between the servers except with collision probability.

\emph{Across attempts.} Attempts run sequentially with fresh preprocessing and a failed check ends the use of $\alpha$, so the per-attempt argument composes sequentially. Without key replacement, the adversary could learn information about $\alpha$ from the pass or fail outcomes of checks it induces, which the per-attempt bound does not account for. \hfill$\square$

